Are Labels Needed for Incremental Instance Learning?

In this paper, we learn to classify visual object instances, incrementally and via self-supervision (self-incremental). Our learner observes a single instance at a time, which is then discarded from the dataset. Incremental instance learning is challenging, since longer learning sessions exacerbate forgetfulness, and labeling instances is cumbersome. We overcome these challenges via three contributions: i. We propose VINIL, a self-incremental learner that can learn object instances sequentially, ii. We equip VINIL with self-supervision to by-pass the need for instance labelling, iii. We compare VINIL to label-supervised variants on two large-scale benchmarks, and show that VINIL significantly improves accuracy while reducing forgetfulness.

==> results.tex <==


\begin{table}[t]
\begin{center}
%\renewcommand{\arraystretch}{1.0}
%\setlength\tabcolsep{14.0pt}
%\begin{sc}
%\begin{adjustbox}{max width=0.5\textwidth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccc}

\toprule 

Method & Supervision & \multicolumn{2}{c}{Core-$50$} & \multicolumn{2}{c}{iLab-$20$M}  \\ 
\midrule 

& & Accuracy (\uparrow) & Forgetting (\downarrow) & Accuracy (\uparrow) & Forgetting (\downarrow) \\  
\midrule 
SGD & Label & 71.450 & 22.436 & 89.340 & 6.500 \\ 
%\cdashlinelr{2-6}
%\rowcolor{LightCyan} SGD  & Self (SimSiam) & 66.068 & 7.826 & 90.247 & 0.000  \\
\rowcolor{LightCyan} SGD & VINIL & \textbf{74.914} & \textbf{4.802} & \textbf{90.398} & \textbf{0.000} \\
%\rowcolor{LightCyan} SGD & Self (SimCLR) & XX & XX & XX & XX \\
\midrule 
Replay & Label & \textbf{88.180} & \textbf{6.741} & 84.464 & 5.696 \\
%\cdashlinelr{2-6}
%\rowcolor{LightCyan} Replay & Self (SimSiam) & 59.208 & 9.680 & 62.707 & 2.694 \\
\rowcolor{LightCyan} Replay & VINIL & 67.677 & 10.095 & \textbf{90.543} & \textbf{0.000} \\
%\rowcolor{LightCyan} Replay & Self (SimCLR) & XX & XX & XX & XX \\
\midrule 
EwC & Label & \textbf{75.117} & 18.268 & 87.690 & 4.535 \\
%\cdashlinelr{2-6}
%\rowcolor{LightCyan} EwC & Self (SimSiam) & 67.511 & 9.716 & 89.509 & 0.000 \\
\rowcolor{LightCyan} EwC & VINIL & 73.011 & \textbf{2.167} & \textbf{90.655} & \textbf{0.000} \\
%\rowcolor{LightCyan} EwC & Self (SimCLR) & XX & XX & XX & XX \\

\bottomrule
\end{tabular} }
%\end{adjustbox}
\end{center}
   \caption{Visual Incremental Instance Learning on Core-$50$~\cite{core50} and iLab-$20$M~\cite{ilab20m}. VINIL outperforms label-supervised variants for $4$ out of $6$ settings, while significantly reducing forgetfulness on both datasets. This indicates self-incremental learning is a strong, label-free alternative to label-supervision.}
  % \end{adjustbox}
\label{tab:category}
\end{table}


\begin{table}[h]
\begin{center}
%\renewcommand{\arraystretch}{1.0}
%\setlength\tabcolsep{14.0pt}
%\begin{sc}
%\begin{adjustbox}{max width=0.5\textwidth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrcccccc}

\toprule 


& Train on$\Longrightarrow$ & Core-$50$ & iLab-$20$M &  &  iLab-$20$M & Core-$50$ \\ 

\cmidrule{3-4}
\cmidrule{6-7}

% & & Core-$50$ & iLab-$20$M  & $\%\Delta$(\downarrow) & iLab-$20$M & Core-$50$ &  $\%\Delta$(\downarrow) \\

 & Test on$\Longrightarrow$  & Core-$50$ & Core-$50$ & &    iLab-$20$M &    iLab-$20$M   \\ 
\cmidrule{3-4}
\cmidrule{6-7}
Method & Supervision & Accuracy  & Accuracy  & $\%\Delta$(\downarrow) & Accuracy & Accuracy  & $\%\Delta$(\downarrow) \\ 
\midrule 
SGD & Label & 71.450 & 59.850 & 16 & 89.340 & 67.249 & 24  \\ 
%\cdashlinelr{2-8}
%\rowcolor{LightCyan} SGD & Self (SimSiam) & 66.068 & 63.423 & \textbf{4} & 90.247 & 72.190 & 25 \\ 
\rowcolor{LightCyan} SGD & VINIL & \textbf{74.914} & \textbf{66.704} & \textbf{10} & \textbf{90.398} & \textbf{76.302} & \textbf{15} \\ 
\midrule 
Replay & Label & \textbf{88.180} & 55.692 & 36 & 84.464 & 69.412 & 17  \\ 
%\cdashlinelr{2-8}

%\rowcolor{LightCyan} Replay & Self (SimSiam) & 59.208 & 49.448 & 16 & 62.707 & 74.145 & 18 \\ 
\rowcolor{LightCyan} Replay & VINIL & 67.677 & \textbf{61.857} & \textbf{8} & \textbf{90.543} & \textbf{76.125} & \textbf{15} \\ 

\midrule 
EwC & Label & \textbf{75.117} & 59.030 & 21 & 87.690 & 70.087 & 20  \\ 
%\cdashlinelr{2-8}

%\rowcolor{LightCyan} EwC & Self (SimSiam) & 67.511 & 67.967 & \textbf{0} & 89.509 & 72.097 & 19 \\

\rowcolor{LightCyan} EwC & VINIL & 73.011 & \textbf{70.648} & \textbf{3} & \textbf{90.655} & \textbf{75.793} & \textbf{16} \\ 

\bottomrule
\end{tabular} }
%\end{adjustbox}
\end{center}
   \caption{Cross-Dataset Generalization on Core-$50$ and iLab-$20$M datasets. VINIL is consistently more robust in cross-dataset generalization when compared with label-supervision. The results indicate that self-supervision improves the generality of visual representations, for instance-incremental setup.}
  % \end{adjustbox}
\label{tab:cross}
\end{table}

 



